A Survey on Query-based API Recommendation

Application Programming Interfaces (APIs) are designed to help developers build software more effectively. Recommending the right APIs for specific tasks has gained increasing attention among researchers and developers in recent years. To comprehensively understand this research domain, we have surveyed to analyze API recommendation studies published in the last 10 years. Our study begins with an overview of the structure of API recommendation tools. Subsequently, we systematically analyze prior research and pose four key research questions. For RQ1, we examine the volume of published papers and the venues in which these papers appear within the API recommendation field. In RQ2, we categorize and summarize the prevalent data sources and collection methods employed in API recommendation research. In RQ3, we explore the types of data and common data representations utilized by API recommendation approaches. We also investigate the typical data extraction procedures and collection approaches employed by the existing approaches. RQ4 delves into the modeling techniques employed by API recommendation approaches, encompassing both statistical and deep learning models. Additionally, we compile an overview of the prevalent ranking strategies and evaluation metrics used for assessing API recommendation tools. Drawing from our survey findings, we identify current challenges in API recommendation research that warrant further exploration, along with potential avenues for future research.

==> Figures/year_paper_cumu.tex <==

\begin{figure}[H]
    \centering
     {\includegraphics[width=0.8\textwidth]{Figures/year_paper_cumu.pdf}}\
     \vspace{-0.1in}
     \caption{The cumulative number of paper published each year from 2012.}
    \label{vuldiag}
\end{figure}


==> Sections/introduction.tex <==
\section{Introduction}
\label{Introduction}

Application programming interfaces (APIs) from official SDKs or third-party libraries are crucial in software development. They package common functionalities as methods for enhanced programming efficiency. With growing software complexity, new APIs are continuously created. For instance, Java JDK Version 16 contains over {4750} modules. The sheer volume of APIs makes it unfeasible for a single developer to fully grasp all before effective software programming. 

In 2009, Zhong et al. introduced MAPO, a bitmap pattern mining algorithm for API usage patterns \cite{zhong2009mapo}. This algorithm retrieves code fragments from an extensive source code knowledge base, based on API method names. Such API usage pattern mining is a fundamental step for API recommendation methods. After years of studying API pattern mining, researchers are now transitioning their attention from API usage pattern mining to automated API recommendations.

Along this line, Heinemann et al. proposed an approach that mines the intentional knowledge embodied in the identifiers of existing
source code and uses an index of this information to recommend API methods based on the code being developed~\cite{heinemann2012identifier}. 
This marked an initial step towards automated API recommendation, inspiring the creation of diverse recommendation tools. %For instance, FOCUS recommends APIs as options for code snippet suggestions~\cite{nguyen2019focus}. These tools can handle both source code and natural language queries effectively.
RACK, developed by Rahman \cite{rahman2016rack}, serves as the pioneering API recommendation tool in addressing natural language programming queries by providing API method names. These tools leverage source code context and historical data. For instance, Zhang et al. introduced RASH \cite{zhang2017recommending} for API recommendations, incorporating API specifications and past issue resolutions. \song{what the connection between these two papers?}

\song{your intro is quite weak, lack of clean motivation and roadmap, can you please read Nima's survey and https://arxiv.org/pdf/2108.09646.pdf to rewrite this?}

While numerous surveys have been proposed for API recommendation, there exists a shortage of systematic reviews in this area\song{which area?}. Such reviews are valuable for providing a comprehensive understanding of API recommendation research. However, existing surveys\song{which survey?} have limitations, particularly in terms of analysis. For example, most reviews concentrate on data collection and evaluation, neglecting the significance of user studies in API recommendation assessment. Additionally, these reviews may not adequately cover recent developments in the field. Compared to existing surveys, this research offers an extensive survey of API recommendation studies, including multiple aspects such as dataset collection, evaluation metrics, models, data representations, knowledge bases, and user studies.

\song{add https://dl.acm.org/doi/abs/10.1145/3628161}

For our review, we gathered \add{72} papers from \add{20} prominent conferences and journals between 2012 and 2023. Initially, we formulated a set of search terms using 10 API recommendation paper titles familiar to our research group. These terms guided our exploration across various paper archive databases. The collected papers underwent manual and automated filtering. Through comprehensive analysis, we address the following research questions (RQs): First, what are the prevailing trends in API recommendation studies? Second, what common components characterize existing API recommendation tools? Third, what are the distinguishing features of current API recommendation tools? Lastly, what evaluation processes are commonly employed in API recommendation research?

\textbf{Contribution.} The contribution of our survey is as follows.
\begin{itemize}

\item As far as our knowledge extends, we are the first to systematically study large-scale API recommendation systems and their subsystems, including data extraction, models, knowledge base restrictions, and evaluation metrics.

\item We believe that we are the pioneers in investigating user studies within the realm of API recommendation. We summarize and categorize the user studies presented in API recommendation papers and draw conclusions based on our analysis.

\item We analyze the challenges inherent in the current state of API recommendation research and provide directions for future API recommendation research endeavors.

\end{itemize}

The paper's structure is as follows: In Section 2, we contextualize the survey by defining software engineering technical terms within the API recommendation research field and offering an overview of a typical API recommendation system's pipeline. Section 3 introduces existing works related to the survey. Section 4 outlines the survey methodology, while Sections 5 to 9 provide detailed insights into each research question and its corresponding answers. In Section 10, we address challenges associated with API recommendation, and Section 11 explores potential opportunities. Section 12 is the conclusion of this study.



==> Sections/limitation.tex <==
\section{limitation}
\label{limitation}

% nebliva: It may be interesting to include a Limitations Section. In that section, you will discuss the limitations of the methods used to conduct the survey and the limitation of the evidence included in the survey. That evidence refers to the data extracted from the surveyed papers.

==> Tables/table_11.tex <==

\begin{table}[h]
\caption{Data type of the collected data sets}
\label{table_11}
\renewcommand{\arraystretch}{0.3}
% \resizebox{\columnwidth}{!}{%/
\begin{tabular}{cll}
\toprule
No & Data Type & Count  \\
\midrule
1   & Code text pair   & 40 \\
2   & Code    & 37 \\
3   & Code and image    & 1 \\
\midrule
    & Total    &  78\\
\bottomrule        
\end{tabular}
% }
\end{table}

==> Tables/table_12.tex <==

\begin{table}[h]
\caption{Data type of the collected data sets}
\label{table_12}
\renewcommand{\arraystretch}{0.3}
% \resizebox{\columnwidth}{!}{%/
\begin{tabular}{cll}
\toprule
No & Data Type & Count  \\
\midrule
1   & Code text pair   & 40 \\
2   & Code    & 37 \\
3   & Code and image    & 1 \\
\midrule
    & Total    &  78\\
\bottomrule        
\end{tabular}
% }
\end{table}

==> Tables/table_13.tex <==
\begin{table}[t!]
\caption{Common API usage extraction methods}
\label{table_13}
\renewcommand{\arraystretch}{0.1}
\begin{tabular}{cll}
\toprule
No & extraction method & Reference      \\
\midrule

1   & Graph analysis   & \cite{nguyen2012grapacc,nguyen2015recommending,chen2021novel,liu2018effective}\\
2   & AST Parsing       & \cite{he2021pyart,yan2018learning,wang2021plot2api}\\
3   & Code Parsing   & \cite{kang2021apirecx,zhao2021icon2code,liu2019autoencoder,ponzanelli2017supporting,liu2019design, wang2021hybrid,tian2018automatically,sun2019enabling,liu2018effective,nguyen2017exploring,raghothaman2016swim,wei2022clear}\\
4   & Document Parsing & \cite{ponzanelli2017supporting, rahman2016rack,lin2018nl2api,yuan2019api,sworna2023apiro,gao2021api,zhang2017recommending,li2020fusion,sun2019enabling,xie2020api,huang2018api,gu2016deep,lee2021mining,wei2022clear}\\




% 1   & Parsing Document  &    \cite{thung2013automatic, ajam2021scout, zhou2021boosting, yin2021api, kim2013enriching, lv2015codehow, xie2020api, huang2018api, hussain2020codegru, yuan2019api}\\
% 2   & AST parser     &  \cite{ling2019graph, zhang2017recommending, rabinovich2017abstract, sun2019enabling, heinemann2012identifier}\\
% 3   & Java Development Tool(JDT)   &  \cite{lee2018comment, gu2019codekernel, tian2018automatically, liu2019accelerating, nguyen2016api, gu2016deep, svyatkovskiy2019pythia, allamanis2013mining, gu2018deep, zhang2016bing, liu2020much, maddison2014structured, liu2018effective, asaduzzaman2015exploring} \\
% 4   & Python AST parse &  \cite{svyatkovskiy2019pythia, wang2021plot2api}\\
% 5   & GrouMiner   & \cite{yin2017syntactic, nguyen2018statistical, nguyen2012grapacc, nguyen2015graph}\\
% 6   & Graph analysis   & \cite{chen2021novel, zhao2021icon2code}\\
% 7   & QA website and online tutorial  & \cite{sun2021task, huang2018api, rahman2016rack, ye2016word}\\
% 8  & regular expression &  \cite{buse2012synthesizing, lu2015query, lee2016categorizing, lee2021mining, monperrus2016searching, campbell2017nlp2code, nie2016query, jiang2016rosf, ye2016word, ling2021graph, asaduzzaman2016simple}\\
% 9  & static analysis &  \cite{nguyen2021recommending, wang2021hybrid, asaduzzaman2017recommending}\\
% 10  & Other tools  & \cite{, liu2019autoencoder, rahman2018effective, asaduzzaman2015exploring, d2016collective, gao2021api}\\
% 11  & NA & \cite{jiang2016rosf, nie2016query, campbell2017nlp2code, zhang2012automatic, chen2021holistic, gvero2015interactive, raychev2014code, richardson2017function, luan2019aroma, chan2012searching, ling2016latent, ponzanelli2017supporting} \\
% % , fucci2019using, allamanis2015bimodal, kang2021apirecx



\bottomrule
\end{tabular}
\end{table}

==> Tables/table_16.tex <==

\begin{table}[h]
\caption{Other modeling techniques}
\label{table_16}
\renewcommand{\arraystretch}{0.3}
\begin{tabular}{clcl}
\toprule
No & extraction method &  Reference      \\
\midrule


2   & graph  model  &\cite{nguyen2015graph, liu2020much, liu2018effective, chan2012searching, ling2019graph, asaduzzaman2017recommending}\\
3   & Latent predictor networks   & \cite{ling2016latent}\\
4   & Learn-to-rank(LTR)  & \cite{zhou2021boosting}\\
5   & Log-bilinear Tree-Traversal Model  & \cite{maddison2014structured}\\
7   & Petri net  & \cite{liu2019accelerating}\\

\bottomrule
\end{tabular}
\end{table}



==> Tables/table_17.tex <==

\begin{table}[h]
\caption{Common Ranking Strategy }
\label{table_17}
\renewcommand{\arraystretch}{0.3}
\begin{tabular}{cll}
\toprule
No & Ranking method & Reference\\
\midrule

1   & Probability &\cite{rahman2016rack,liu2019autoencoder,allamanis2015bimodal,yin2021api,lv2015codehow,wang2021hybrid}\\
& &\cite{tian2018automatically,chen2021novel,chen2021holistic,kang2021apirecx}\\
& &\cite{asaduzzaman2017recommending,nguyen2015graph,hussain2020codegru,nguyen2016learning}\\
& &\cite{ling2016latent,svyatkovskiy2019pythia,allamanis2013mining,richardson2017function}\\
& &\cite{gvero2015interactive,raychev2014code,gu2016deep,campbell2017nlp2code}\\
& &\cite{fucci2019using,wang2021plot2api,gu2018deep,liu2019design,liu2019accelerating}\\
2   & Heuristic  &\cite{nguyen2016api,heinemann2012identifier,lee2021mining,rahman2018effective,gu2019codekernel,liu2018effective,ling2019graph,nguyen2018statistical}\\
& &\cite{xie2019hirec,zhang2012automatic,d2016collective,sun2021task,zhou2021boosting,maddison2014structured,he2021pyart,nie2016query,huang2018api,jiang2016rosf,zhang2017recommending}\\
3   & Similarity &\cite{yuan2019api,nguyen2021recommending,sun2019enabling,liu2020much,raghothaman2016swim,zhao2021icon2code,ajam2021scout,gao2021api,thung2013automatic,ye2016word,luan2019aroma,ponzanelli2017supporting,lu2015query,xie2020api}\\

\bottomrule
\end{tabular}
\end{table}



==> Tables/table_19.tex <==

\begin{table}[h]
\caption{List of Studies Considering User Study }
\label{table_19}
% \renewcommand{\arraystretch}{0.1}
\begin{tabular}{llllll}
\toprule
Paper & participants & \#tasks & tasks type & evaluation method      \\


\midrule

Wang et al.\cite{wang2014active} & 10 students & 10 & grading the relevance & NDCG\\

Xie et al.\cite{xie2020api} & 12 students & 30  & select correct API & Accuracy\\

Huang et al.\cite{huang2018api} & 28 developers & 10 & search solution & Correctness, Time \\
 
Luan et al.\cite{luan2019aroma} & 12 developers & 4 & write code & Correctness \\

zhang et al.\cite{zhang2012automatic} & 8 students & 2 & fill in missing APIs & Questionnaire\\

zhang et al.\cite{zhang2016bing} & 1 developer & 150 & label relevancy & MRR\\

Lv et al.\cite{lv2015codehow} & 20 developers & 3 & search solution & Relevancy\\

Gu et al.\cite{gu2019codekernel} & 20 developers & 10 & search solution & Representativeness \\

Chen et al.\cite{chen2021holistic} & 18 students & 6 & search solution & Time, Accuracy\\

Nguyen et al.\cite{nguyen2021recommending} & 16 students & 2 & write code & Success rate\\

Nguyen et al.\cite{nguyen2018statistical} & 4 developers & 5 & grading generated result & Usefulness\\

Ponzanelli et al.\cite{ponzanelli2017supporting} & 16 students & 4 & write code& Questionnaire\\

Buse et al.\cite{buse2012synthesizing} & 25 students & 35 & choose preferred options & Grading 1-6\\

Sun et al.\cite{sun2021task} & 12 students & 6 & bug-fixing with API & Usefulness\\

\bottomrule
\end{tabular}
\end{table}



==> Tables/table_2.tex <==
\begin{table}[h]
\caption{Comparison of related work }
\label{table_2}
\renewcommand{\arraystretch}{0.1}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cl}
\toprule
Decision &Criteria \\
\midrule
  RQ1 & Years, Conference, application direction, common keywords. \\
  RQ2 & Data source, language, API libraries, data type, \\
      & data size, API extraction strategy, Ground truth extraction strategy. \\
  RQ3 & models, application, motivation, ranking strategy. \\
  RQ4 & Test data size, Test data type, evaluation metric, human factor. \\
\bottomrule
\end{tabular}%
}
\end{table}



==> Tables/table_21.tex <==

\begin{table}[h]
\caption{Comparison of related work }
\label{table_20}
% \renewcommand{\arraystretch}{0.1}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Paper & data collection & evaluation metric & model & representation & knowledge base & user study\\
\midrule
Peng et al.\cite{peng2022revisiting}      & \checkmark & \checkmark  &            &            &            &           \\
Allamanis et al.\cite{allamanis2018survey}& \checkmark & \checkmark  & \checkmark & \checkmark &            &           \\
Liu et al.\cite{liu2021opportunities}     & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark &           \\ 
Ours                                      & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark & \checkmark\\

\bottomrule
\end{tabular}%
}
\end{table}



==> Tables/table_3.tex <==
\begin{table}[h]
\caption{Inclusion and exclusion keywords in paper titles and abstract.}
\label{table_3}
% \renewcommand{\arraystretch}{0.1}
{%
\begin{tabular}{|l|l|}
  \hline			
  Conference & 68 \\
  \hline
  Journal & 21 \\
  \hline 
% \bottomrule
\end{tabular}}
\end{table}

==> Tables/table_4.tex <==
\begin{table}[h]
\caption{Inclusion and exclusion keywords in paper titles and abstract.}
\label{table_4}
% \renewcommand{\arraystretch}{0.1}
{%
\begin{tabular}{|l|l|}
\hline
ICSE & 17 \\
\hline
ASE & 6 \\
\hline
FSE & 7 \\
\hline
ICSME & 8 \\
\hline
TSE & 4 \\
\hline
SANER & 4 \\
\hline
arXiv & 4  \\
\hline 
IEEE Access & 3 \\
\hline
IST & 3  \\
\hline 
MSR & 3  \\
\hline 
QRS & 2 \\
\hline
PLMR & 2  \\
\hline 
APSEC & 1  \\
\hline 
CASCON & 1  \\
\hline 
CLEI & 1  \\
\hline 
COMPSAC & 1  \\
\hline 
JCST & 1  \\
\hline 
CSMR & 1  \\
\hline 
EMNLP & 1  \\
\hline 
ICCSE & 1  \\
\hline 
ICS & 1  \\
\hline 
IET & 1  \\
\hline 
ISSRE & 1  \\
\hline 
ISSTA & 1  \\
\hline 
JIT & 1  \\
\hline 
JPCS & 1  \\
\hline 
JSEP & 1  \\
\hline 
ICWS & 1 \\
\hline
OOPSLA & 1  \\
\hline 
PLDI & 1  \\
\hline 
SCAM & 1  \\
\hline 
SCIS & 1  \\
\hline 
SCP & 1  \\
\hline 
SIGKDD & 1  \\
\hline 
TETCI & 1  \\
\hline 
TOIS & 1  \\
\hline 
TOSEM & 1  \\
\hline 
TSC & 1  \\
\hline 
% \bottomrule
\end{tabular}}
\end{table}

==> Tables/table_4_1.tex <==
\begin{table}[h]
\caption{Conference publication venues for manual search}
\label{table_9}
\renewcommand{\arraystretch}{0.1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll}
\toprule
Conference & count   \\
\midrule
ICSE & 17 \\
ASE & 6 \\
FSE & 7 \\
ICSME & 8 \\
TSE & 4 \\
SANER & 4 \\
arXiv & 4  \\
IEEE Access & 3 \\
IST & 3  \\
MSR & 3  \\
QRS & 2 \\
PLMR & 2  \\
Others & 26  \\
\bottomrule
\end{tabular}}
\end{table}

==> Tables/table_5.tex <==
\begin{table}[h]
\caption{Inclusion and exclusion keywords in paper titles and abstract.}
\label{table_5}
% \renewcommand{\arraystretch}{0.1}
{%
\begin{tabular}{|l|l|}
\hline
year & number of publication\\
\hline
2012 & 6 \\
\hline
2013 & 4 \\
\hline
2014 & 5 \\
\hline
2015 & 7 \\
\hline
2016 & 16 \\
\hline
2017 & 11 \\
\hline
2018 & 7 \\
\hline
2019 & 13 \\
\hline
2020 & 7 \\
\hline
2021 & 14 \\
\hline
Total & 90 \\
\hline
% \bottomrule
\end{tabular}}
\end{table}

==> Tables/table_5_1.tex <==
\begin{table}[h]
\caption{Inclusion and exclusion keywords in paper titles and abstract.}
\label{table_5_1}
% \renewcommand{\arraystretch}{0.1}
{%
\begin{tabular}{|l|l|}
\hline
year & number of accumulative publication \\
\hline
2012 & 6\\
\hline
2013 & 10\\
\hline
2014 & 15\\
\hline
2015 & 22\\
\hline
2016 & 38\\
\hline
2017 & 49\\
\hline
2018 & 56\\
\hline
2019 & 69\\
\hline
2020 & 76\\
\hline
2021 & 90 \\
\hline
% \bottomrule
\end{tabular}}
\end{table}

==> Tables/table_5_2.tex <==
\begin{table}[h]
\caption{Inclusion and exclusion keywords in paper titles and abstract.}
\label{table_5_2}
% \renewcommand{\arraystretch}{0.1}
{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
year & publication & Recommendation & completion & generation & other \\
\hline
2012 & 3 & 1 & 0 & 2 & 0\\
\hline
2015 & 2 & 2 & 0 & 0 & 0\\
\hline
2016 & 7 & 5 & 0 & 1 & 1\\
\hline
2017 & 3 & 2 & 0 & 0 & 1\\
\hline
2018 & 5 & 3 & 0 & 1 & 1\\
\hline
2019 & 10 & 6 & 0 & 1 & 3\\
\hline
2020 & 6 & 4 & 1 & 1 & 0\\
\hline
2021 & 14 & 7 & 3 & 2 & 2\\
\hline
total & 50 & 30 & 4 & 8 & 8\\
\hline
% \bottomrule
\end{tabular}}
\end{table}

==> Tables/table_6.tex <==
\begin{table}[h]
\caption{Inclusion and exclusion keywords in paper titles and abstract.}
\label{table_6}
% \renewcommand{\arraystretch}{0.1}
{%
\begin{tabular}{|l|l|}
\hline
Heuristics & 15 \\
\hline
Deep Learning & 19 \\
\hline
Knowledge Graph & 11 \\
\hline
Machine learning & 8 \\
\hline
% \bottomrule
\end{tabular}}
\end{table}

==> Tables/table_7.tex <==
\begin{table}[h]
\caption{Inclusion and exclusion keywords in paper titles and abstract.}
\label{table_7}
% \renewcommand{\arraystretch}{0.1}
{%
\begin{tabular}{|l|l|}
\hline
Github & 24 \\
\hline
Stack Overflow & 13 \\
\hline
other & 11 \\
\hline
% \bottomrule
\end{tabular}}
\end{table}

==> Tables/table_8.tex <==

\begin{table}[h]
\caption{Data type of the collected data sets}
\label{table_8}
\renewcommand{\arraystretch}{0.3}
% \resizebox{\columnwidth}{!}{%/
\begin{tabular}{cll}
\toprule
No & Data Type & Count  \\
\midrule
1   & Code {\&} text pair   & 38  \\
2   & API call sequence     & 12 \\
3   & Partial Source code   & 11  \\
4   & Graph                 & 7  \\
5   & Abstract Syntax Tree  & 6 \\
6   & Source code           & 3  \\
7   & Image                 & 1  \\
\midrule

   & Total                 & 72  \\
\bottomrule        
\end{tabular}
% }
\end{table}
